Bellman Eluder Dimension: New Rich Classes of RL Problems, and Sample-Efficient Algorithms

Finding the minimal structural assumptions that empower sample-efficient learning is one of the most important research directions in Reinforcement Learning (RL). This paper advances our understanding of this fundamental question by introducing a new complexity measure -- Bellman Eluder (BE) dimension. We show that the family of RL problems of low BE dimension is remarkably rich, which subsumes a vast majority of existing tractable RL problems including but not limited to tabular MDPs, linear MDPs, reactive POMDPs, low Bellman rank problems as well as low Eluder dimension problems. This paper further designs a new optimization-based algorithm -- GOLF, and reanalyzes a hypothesis elimination-based algorithm -- OLIVE (proposed in Jiang et al., 2017). We prove that both algorithms learn the near-optimal policies of low BE dimension problems in a number of samples that is polynomial in all relevant parameters, but independent of the size of state-action space. Our regret and sample complexity results match or improve the best existing results for several well-known subclasses of low BE dimension problems.

==> pfoverview.tex <==
\subsection{An alternative way to define \be\ dimension}

Define $\|\Fcal\|_{\infty}=\sup_{f\in\Fcal}\|f\|_{\infty}$.
\begin{definition}[\textsf{BEN} dimension]
	Given a function class $\Fcal$ defined on $\Xcal$ and a distribution family $\Pi$ over $\Xcal$. 
	Define \bendim$(\Fcal,\Pi,T)$ to be the smallest $d\in\N$ such that: for all $\beta\ge\|\Fcal\|_{\infty}^2$ as well as $f_1,\ldots,f_T\in\Fcal$ and $\mu_1,\ldots,\mu_T\in\Pi$, if ${\sum_{i<t}\E_{\mu_i}[f_t^2]}\le \beta$ holds for all $t\in[T]$, then $\sum_{t=1}^{T} \E_{\mu_t}[f_t]\le \sqrt{d\beta T}$.
\end{definition}


The following two lemmas hold for arbitrary $\Fcal$ and $\Pi$.
\begin{lemma}
	\bendim$(\Fcal,\Pi,T)\le\Ocal(\dedim (\Fcal,\Pi,1/T^2))$.
\end{lemma}
\begin{proof}
	To begin with, note that 
	${\sum_{i<t}(\E_{\mu_i}[f_t])^2}\le {\sum_{i<t}\E_{\mu_i}[f_t^2]}\le \beta$. So we can apply lemma \ref{lem:de-regret} and obtain
	$$
	\sum_{t=1}^{T} \E_{\mu_t} [f_t] \le \Ocal\left(\sqrt{\dedim (\Fcal,\Pi,1/T^2)\beta T}\right),
	$$
	which immediately implies \bendim$(\Fcal,T)\le\Ocal(\dedim (\Fcal,\Pi,1/T^2))$.
\end{proof}

\begin{lemma}
	\bendim$(\Fcal,\Pi,T)\le \Ocal(\dedim (\Fcal,\Dcal_{\dirac},1/T^2)\log(T))$.
\end{lemma}
\begin{proof}
Sample $x_1,\ldots,x_T$ independently and respectively from $\mu_1,\ldots,\mu_T$. 

By Bernstein inequality, with probability at least $3/4$, we have for all $t\in[T]$,
\begin{equation}
\begin{aligned}
	\sum_{i<t}(f_t(x_i))^2
\le &\Ocal\paren{\sqrt{(\sum_{i<t}\E_{\mu_i}[f_t^4])\log T}+ \|\Fcal\|_{\infty}^2\log T}\\
	\le &\Ocal\paren{\|\Fcal\|_{\infty}^2 \sqrt{(\sum_{i<t}\E_{\mu_i}[f_t^2])\log T}+ \|\Fcal\|_{\infty}^2\log T}\\
	\le &\Ocal\paren{\|\Fcal\|_{\infty}^2 \sqrt{\beta\log T}+ \|\Fcal\|_{\infty}^2\log T}
\le  \Ocal\paren{\beta\log T}.
\end{aligned}
\end{equation}
By Hoeffding's inequality, with probability at least $3/4$, we have
\begin{equation}
\begin{aligned}
\sum_{t=1}^{T} \E_{\mu_t} [f_t] \le
\sum_{t=1}^{T} f_t(x_t) + \Ocal(\|\Fcal\|_\infty \sqrt{T})
\le \sum_{t=1}^{T} f_t(x_t) +  \Ocal(\sqrt{T\beta}).
\end{aligned}
\end{equation}
By taking a union bound, we have with positive probability, $\sum_{i<t}(f_t(x_i))^2\le \Ocal\paren{\beta\log T}$ for all $t\in[T]$ and 
$\sum_{t=1}^{T} \E_{\mu_t} [f_t]\le \sum_{t=1}^{T} f_t(x_t) +  \Ocal(\sqrt{T\beta})$. Now we can apply lemma \ref{lem:de-regret} and obtain
$$
\sum_{t=1}^{T} \E_{\mu_t} [f_t] \le 
\sum_{t=1}^{T} f_t(x_t) +  \Ocal(\sqrt{T\beta})
\le \Ocal\left(\sqrt{\dedim (\Fcal,\Dcal_{\dirac},1/k^2)\log(T)\beta T } \right),
$$
which immediately implies \bendim$(\Fcal,T)\le\Ocal(\dedim (\Fcal,\Dcal_{\dirac},1/T^2)\log(T))$.
\end{proof}











	
	
